Representation Learning on Heterophilic Graph with Directional Neighborhood Attention

Graph Attention Network (GAT) is one of the most popular Graph Neural Network (GNN) architecture, which employs the attention mechanism to learn edge weights and has demonstrated promising performance in various applications. However, since it only incorporates information from immediate neighborhood, it lacks the ability to capture long-range and global graph information, leading to unsatisfactory performance on some datasets, particularly on heterophilic graphs. To address this limitation, we propose the Directional Graph Attention Network (DGAT) in this paper. DGAT is able to combine the feature-based attention with the global directional information extracted from the graph topology. To this end, a new class of Laplacian matrices is proposed which can provably reduce the diffusion distance between nodes. Based on the new Laplacian, topology-guided neighbour pruning and edge adding mechanisms are proposed to remove the noisy and capture the helpful long-range neighborhood information. Besides, a global directional attention is designed to enable a topological-aware information propagation. The superiority of the proposed DGAT over the baseline GAT has also been verified through experiments on real-world benchmarks and synthetic data sets. It also outperforms the state-of-the-art (SOTA) models on 6 out of 7 real-world benchmark datasets.

==> env.tex <==
% My macros
\ProvidesPackage{mymacros}
% 23/4/99 version of shtrpt2.tex.
\usepackage{latexsym}   
\usepackage{bm}
\usepackage{verbatim}
%\usepackage[final]{graphicx}
%\usepackage{labmat}
%\usepackage{algorithmic}

%\usepackage{algorithmic}
%\usepackage{algpseudocode}


%\usepackage{algorithm}
%\usepackage[sectionbib]{natbib}
%\usepackage{chapterbib}
%\usepackage[showframe]{geometry}
\usepackage{color}
\usepackage{enumitem}
\usepackage{amsthm}
%\setcounter{secnumdepth}{3}

% Define \br or \bl may cause troubles.
%
% Very large page format:
%\addtolength{\textheight}{2in}
%\addtolength{\textwidth}{2.6in}
%\addtolength{\oddsidemargin}{-1.5in}
%\addtolength{\topmargin}{-1.2in}
%\renewcommand{\baselinestretch}{1}

% Large page format that Xiao-Wen was using:
%\textwidth=17.5cm
%\textheight=23.9cm
%\oddsidemargin=-16pt
%\topmargin=-55pt

%\parskip=5pt plus 1pt minus 1pt


% New Commands.

% Theorem-like environments (Ray's):
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{lemma}{Lemma}[section]
%\newtheorem{proposition}{Proposition}[section]
%\newtheorem{definition}{Definition}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]
%\renewcommand{algorithm}{lgorithm}[section]



%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}


%\renewcommand{\abstractname}{Summary}
% Spaces
\newcommand{\noi}{\noindent}
\newcommand{\hsp}{\hspace}
\newcommand{\vsp}{\vspace}
\renewcommand{\top}{{\mkern-1.5mu\mathsf{T}}}

% Equations:
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqy}{\begin{eqnarray}}
\newcommand{\eeqy}{\end{eqnarray}}
\newcommand{\beqynn}{\begin{eqnarray*}}
\newcommand{\eeqynn}{\end{eqnarray*}}

% Arrays, Matrices and Tables:
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
% For a matrix:
\newcommand{\bmx}{\begin{bmatrix}}
\newcommand{\emx}{\end{bmatrix}}
\newcommand{\bsmx}{\left[\begin{smallmatrix}}
\newcommand{\esmx}{\end{smallmatrix}\right]}
\newcommand{\bmxc}[1]{\left[\begin{array}{@{}#1@{}}}
\newcommand{\emxc}{\end{array}\right]}
% example: \bmx{@{}c@{}c@{}c@{}} 1 & 0 & 0 \\ 0 & 1 & 0 \\ 0 & 0 & 1 \emx
%         denotes a very thin 3 by 3 identity matrix.

% Tables have a similar format:
\newcommand{\bt}[1]{\begin{tabular}{#1}}
\newcommand{\et}{\end{tabular}}
% eg \bt{lrc} Name & Mark & Grade \\ \hline Emma Winner & 99 & A+ \et

% Displays:
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}

% Statistical Material:
\newcommand{\prob}[1]{P\{ #1 \} }
\newcommand{\Exp}[1]{\mathrm{E}\!\left\{#1 \right\}}
\newcommand{\cov}[1]{\mathrm{cov}\!\left\{#1\right\}}
\newcommand{\var}[1]{\mathrm{var}\{#1\}}
\newcommand{\pfd}{\mathcal{P}_{\mathrm{fd}}}
\newcommand{\tfd}{\theta_{\mathrm{fd}}}
\newcommand{\pmd}{\mathcal{P}_{\mathrm{md}}}
\newcommand{\pfi}{\mathcal{P}_{\mathrm{fi}}}
\newcommand{\tfi}{\theta_{\mathrm{fi}}}
\newcommand{\sign}{\mathrm{sgn}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\relu}{\mathrm{ReLU}}
\newcommand{\cost}{\mathrm{cost}}
\newcommand{\diver}{\mathrm{div}}
\newcommand{\leakyrelu}{\mathrm{LeakyReLU}}
\newcommand{\agg}{\mathrm{AGGREGATE}}
\newcommand{\update}{\mathrm{UPDATE}}
\newcommand{\att}{\mathrm{att}}
\newcommand{\clear}[1]{\mathrel{\raisebox{-.75ex}{$#1$}}}
% use: \hline \clear{\bar{b}}
\usepackage{scalerel}




% Instead of \equiv could use engineer's:
%\newcommand{\defn}{\mathrel{\raisebox{-.75ex}{$\mathop{=}\limits^{\triangle}$}}}
\newcommand{\defn}{\triangleq}
% Approx
\newcommand{\alt}{\mathrel{\raisebox{-.75ex}{$\mathop{\sim}\limits^{\textstyle <}$}}}
% instead of
%\begin{array}{c} \\ \stackrel{\textstyle<}{\sim}\vspace{2mm}\end{array}

% Styles
\newcommand{\sss}{\scriptscriptstyle}
\newcommand{\sR}{{\sss R}}
\newcommand{\sS}{{\sss S}}
\newcommand{\sLS}{{\sss  \mathrm{LS}}}
\newcommand{\sILS}{{\sss  \mathrm{ILS}}}
\newcommand{\sTLS}{{\sss  \mathrm{TLS}}}
\newcommand{\sTSVD}{{\sss  \mathrm{TSVD}}}
\newcommand{\sBlockILS}{{\sss  \mathrm{BOB}}}
\newcommand{\stwoblockBabai}{{\sss  \mathrm{BOB2}}}
\newcommand{\sBlockBabai}{{\sss  \mathrm{BOB}}}
\newcommand{\sBOB}{{\sss  \mathrm{BOB}}}
\newcommand{\sRB}{{\sss  \mathrm{RB}}}
\newcommand{\snew}{{\sss  \mathrm{NEW}}}
\newcommand{\sBOR}{{\sss  \mathrm{BOR}}}
\newcommand{\spp}{{\sss  \mathrm{p}}}
\newcommand{\scc}{{\sss  \mathrm{c}}}
\newcommand{\sidx}{{\sss  \mathrm{Id}}}
\newcommand{\sKB}{{\sss  \mathrm{B_{\scaleto {KL}{3pt}}}}}
\newcommand{\sKBone}{{\sss  \mathrm{B_{\scaleto {K1}{3pt}}}}}
\newcommand{\sKfiveBone}{{\sss  \mathrm{B_{\scaleto {5,1}{4pt}}}}}
\newcommand{\sRBK}{{\sss  \mathrm{RB_{\scaleto {K}{3pt}}}}}
\newcommand{\srls}{{\sss  \mathrm{RLS}}}
\newcommand{\sBOBS}{{\sss  \mathrm{BOBS}}}
\newcommand{\sDL}{{\sss  \mathrm{DL}}}
\newcommand{\sDLL}{{\sss  \mathrm{DL2}}}
\newcommand{\sDLLL}{{\sss  \mathrm{DL}}}
\newcommand{\sFSD}{{\sss  \mathrm{FCSD}}}
% Symbols and  mathematical functions:
%\newcommand{\det}{\mathrm{det}} % this is already defined, somewhere in latex
%\renewcommand{\span}{\mathrm{span}} % this is already defined, somewhere in latex
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\trace}{\mathrm{trace}}
\newcommand{\erf}{\mathrm{erf}}
\newcommand{\schi}{{\sss  \mathrm{Chi}}}
\newcommand{\sest}{{a}}
\newcommand{\dist}{\mathrm{dist}}
\newcommand{\schisq}{{\sss  \mathrm{Chi-Sq}}}
\newcommand{\al}[1]{\begin{align}#1\end{align}}
\newcommand{\aln}[1]{\begin{align*}#1\end{align*}}


\newcommand{\eps}{\epsilon}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}


% dimension fo physical quantities:
\newcommand{\Hz}{\mathrm{Hz}}
\newcommand{\KHz}{\mathrm{KHz}}
\newcommand{\MHz}{\mathrm{MHz}}
\newcommand{\GHz}{\mathrm{GHz}}
\newcommand{\km}{\mathrm{km}}
\newcommand{\cm}{\mathrm{cm}}
\newcommand{\chips}{\mathrm{chips}}
\newcommand{\Megachips}{\mathrm{Mega-chips}}


\newcommand{\Rbb}{{\mathbb{R}}}
\newcommand{\Zbb}{{\mathbb{Z}}}
\newcommand{\Cbb}{{\mathbb{C}}}

\newcommand{\kbk}{{k \times k}}
\newcommand{\nbk}{{n \times k}}
\newcommand{\nbn}{{n \times n}}
\newcommand{\nbm}{{n \times m}}
\newcommand{\nbp}{{n \times p}}
\newcommand{\mbm}{{m \times m}}
\newcommand{\mbn}{{m \times n}}
\newcommand{\mbp}{{m \times p}}
\newcommand{\pbn}{{p \times n}}
\newcommand{\pbp}{{p \times p}}
\newcommand{\mbmmn}{{m \times (m-n)}}

\newcommand{\Rk}{\Rbb^{k}}
\newcommand{\Rm}{\Rbb^{m}}
\newcommand{\Rn}{\Rbb^{n}}
\newcommand{\Rp}{\Rbb^{p}}
\newcommand{\Rkbk}{\Rbb^{k \times k}}
\newcommand{\Rnbk}{\Rbb^{n \times k}}
\newcommand{\Rnbn}{\Rbb^{n \times n}}
\newcommand{\Rnbm}{\Rbb^{n \times m}}
\newcommand{\Rnbp}{\Rbb^{n \times p}}
\newcommand{\Rmbm}{\Rbb^{m \times m}}
\newcommand{\Rmbn}{\Rbb^{m \times n}}
\newcommand{\Rmbk}{\Rbb^{m \times k}}
\newcommand{\Rmbp}{\Rbb^{m \times p}}
\newcommand{\Rpbn}{\Rbb^{p \times n}}
\newcommand{\Rpbm}{\Rbb^{p \times m}}
\newcommand{\Rpbp}{\Rbb^{p \times p}}
\newcommand{\Rmbmmn}{\Rbb^{m \times (m-n)}}
\newcommand{\Cn}{\Cbb^{n}}
\newcommand{\Cmbn}{\Cbb^{m\times n}}
\newcommand{\Zm}{\Zbb^{m}}
\newcommand{\Zn}{\Zbb^{n}}
\newcommand{\Zmbn}{\Zbb^{m \times n}}
\newcommand{\Znbn}{\Zbb^{n \times n}}

% Special for this paper:
\newcommand{\la}{\lambda}
%\newcommand{\N}{\nabla}
%\newcommand{\D}{\Delta}
\newcommand{\hbeta}{\hat{\beta}}
\newcommand{\hrho}{\hat{\rho}}
%\newcommand{\br}{\bar{r}}
\newcommand{\hiav}{\hat{\iav}}
\newcommand{\tiav}{\tilde{\iav}}
%\newcommand{\bl}{x_b}
\newcommand{\sd}{s}
\newcommand{\dd}{d}
\newcommand{\td}{t}
\newcommand{\dr}{\delta_R}
\newcommand{\ds}{\delta_S}
\newcommand{\dt}{\delta_T}
\newcommand{\ecm}{\bSigma}
\newcommand{\mnc}{\bSigma}
\newcommand{\pnc}{\bSigma} 
\newcommand{\pmat}{Q_2^T}
\newcommand{\pvec}{p}
\newcommand{\hs}{\hat{\sigma}}
\newcommand{\ia}{\alpha}
\newcommand{\iaij}{\alpha^{i,j}}
\newcommand{\iav}{\boldsymbol{a}}
\newcommand{\DD}{{\sss DD}}
\newcommand{\SD}{{\sss SD}}


\newcommand{\A}{\mathbf{A}}
\newcommand{\B}{\mathbf{B}}
\newcommand{\C}{\mathbf{C}}
\newcommand{\D}{\mathbf{D}}
\newcommand{\E}{\mathbf{E}}
\newcommand{\F}{\mathbf{F}}
\newcommand{\G}{\mathbf{G}}
\renewcommand{\H}{\mathbf{H}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\J}{\mathbf{J}}
\newcommand{\K}{\mathbf{K}}
\renewcommand{\L}{\mathbf{L}}
\newcommand{\M}{\mathbf{M}}
\newcommand{\N}{\mathbf{N}}
\renewcommand{\P}{\mathbf{P}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\R}{\mathbf{R}}
\newcommand{\boldS}{\mathbf{S}}
\newcommand{\T}{\mathbf{T}}
\newcommand{\U}{\mathbf{U}}
\newcommand{\V}{\mathbf{V}}
\newcommand{\W}{\mathbf{W}}
\newcommand{\X}{{\mathbf{X}}}
\newcommand{\Y}{{\mathbf{Y}}}
\newcommand{\Z}{\mathbf{Z}}

\newcommand{\hbR}{\hat{\R}}


\renewcommand{\a}{\mathbf{a}}
\renewcommand{\b}{\mathbf{b}}
\renewcommand{\c}{\mathbf{c}}
\renewcommand{\d}{\mathbf{d}}
\newcommand{\e}{\mathbf{e}}
\newcommand{\f}{\mathbf{f}}
\newcommand{\g}{\mathbf{g}}
\newcommand{\h}{\mathbf{h}}
\newcommand{\m}{\mathbf{m}}
\renewcommand{\l}{\mathbf{l}}
\newcommand{\n}{\mathbf{n}}
\newcommand{\p}{\mathbf{p}}
\newcommand{\q}{\mathbf{q}}

\newcommand{\boldr}{\mathbf{r}}
%\renewcommand{\r}{\mathbf{r}}

\newcommand{\s}{\mathbf{s}}
\newcommand{\boldt}{\mathbf{t}}

\renewcommand{\u}{\mathbf{u}}
\renewcommand{\v}{{\mathbf{v}}}

\newcommand{\w}{{\mathbf{w}}}
\newcommand{\x}{{\mathbf{x}}}
\newcommand{\y}{{\mathbf{y}}}
\newcommand{\z}{{\mathbf{z}}}

\newcommand{\phib}{\bm{\phi}}
\newcommand{\lambdab}{\bm{\lambda}}


\newcommand{\bSigma}{{\boldsymbol{\Sigma}}}
\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bbSigma}{{\bar{\bSigma}}}

\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bnu}{\boldsymbol{\nu}}
\newcommand{\boldeta}{\boldsymbol{\eta}}


\newcommand{\0}{{\boldsymbol{0}}}
\newcommand{\1}{{\boldsymbol{1}}}
\newcommand{\binfty}{{\boldsymbol{\infty}}}


\newcommand{\bd}{{\bar{d}}}
%\newcommand{\bl}{{\bar{l}}}
%\newcommand{\br}{{\bar{r}}}
\newcommand{\bx}{{\bar{x}}}
\newcommand{\by}{{\bar{y}}}
\newcommand{\bz}{{\bar{z}}}
\newcommand{\bE}{{\bar{E}}}

\newcommand{\bbA}{\boldsymbol{\bar{A}}}
\newcommand{\bbD}{\boldsymbol{\bar{D}}}
\newcommand{\bbG}{\boldsymbol{\bar{G}}}
\newcommand{\bbL}{\boldsymbol{\bar{L}}}
\newcommand{\bbP}{\boldsymbol{\bar{P}}}
\newcommand{\bbQ}{\boldsymbol{\bar{Q}}}
\newcommand{\bbR}{\boldsymbol{\bar{R}}}

\newcommand{\bbb}{{\bar{\b}}}
\newcommand{\bbc}{{\bar{\c}}}
\newcommand{\bbq}{{\bar{\q}}}
\newcommand{\bbx}{{\bar{\x}}}
\newcommand{\bby}{{\bar{\y}}}
\newcommand{\bbz}{{\bar{\z}}}
\newcommand{\bbu}{{\bar{\u}}}
\newcommand{\bbv}{{\bar{\v}}}

\newcommand{\cbC}{{\check{\C}}}
\newcommand{\cbc}{{\check{\c}}}
\newcommand{\cbu}{{\check{\u}}}
\newcommand{\cbx}{{\check{\x}}}
\newcommand{\cby}{{\check{\y}}}
\newcommand{\cbg}{{\check{\g}}}
\newcommand{\cbv}{{\check{\v}}}

\newcommand{\cA}{{\mathcal{A}}}
\newcommand{\cN}{{\mathcal{N}}}
\newcommand{\cR}{{\mathcal{R}}}

\newcommand{\hb}{\hat{b}}
\newcommand{\hx}{\hat{x}}
\newcommand{\hr}{\hat{r}}
\newcommand{\hy}{\hat{y}}
\newcommand{\hz}{\hat{z}}

\newcommand{\hbE}{{\hat{\E}}}
\newcommand{\hbG}{{\hat{\G}}}
\newcommand{\hbc}{{\hat{\c}}}
\newcommand{\hbd}{{\hat{\d}}}
\newcommand{\hbr}{{\hat{\boldr}}}
\newcommand{\hbv}{{\hat{\v}}}
\newcommand{\hbx}{{\hat{\x}}}
\newcommand{\hby}{{\hat{\y}}}
\newcommand{\hbz}{{\hat{\z}}}
\newcommand{\hbw}{{\hat{\w}}}

\newcommand{\hhbx}{{\hat{\hbx}}}
\newcommand{\hbb}{{\hat{\b}}}

\newcommand{\tl}{\tilde{l}}
\newcommand{\tu}{\tilde{u}}
\newcommand{\tx}{\tilde{x}}
\newcommand{\tv}{\tilde{v}}
\newcommand{\ty}{\tilde{y}}
\newcommand{\tz}{\tilde{z}}


\newcommand{\tbA}{{\tilde{\A}}}
\newcommand{\tbJ}{{\boldsymbol{\tilde{J}}}}
\newcommand{\tbQ}{{\tilde{\Q}}}
\newcommand{\tbR}{{\tilde{\R}}}
\newcommand{\tbL}{{\tilde{\L}}}
\newcommand{\tbU}{{\tilde{\U}}}


\newcommand{\tbl}{{\tilde{\l}}}
\newcommand{\tbu}{{\tilde{\u}}}

\newcommand{\tbp}{{\tilde{\p}}}
\newcommand{\tbq}{{\tilde{\q}}}
\newcommand{\tbv}{{\tilde{\v}}}
\newcommand{\tbw}{{\tilde{\w}}}
\newcommand{\tbx}{{\tilde{\x}}}
\newcommand{\tby}{{\tilde{\y}}}
\newcommand{\tbz}{{\tilde{\z}}}

\newcommand{\vbx}{\vec{\x}}
\newcommand{\vbg}{\vec{\g}}
\newcommand{\vby}{\vec{\y}}


% Special symbols:

\newcommand{\rw}{{\mathrm{rw}}}
\newcommand{\sym}{{\mathrm{sym}}}
\newcommand{\ind}{{\mathrm{ind}}}

\newcommand{\sA}{{\scriptscriptstyle A}}
\newcommand{\sE}{{\scriptscriptstyle E}}
%\newcommand{\sLS}{{\scriptscriptstyle \text{LS}}}
%\newcommand{\sILS}{{\scriptscriptstyle \text{ILS}}}
\newcommand{\sRLS}{{\scriptscriptstyle \mathrm{RLS}}}
\newcommand{\sOL}{{\scriptscriptstyle \mathrm{OL}}}
\newcommand{\sOB}{{\scriptscriptstyle \mathrm{OB}}}
\newcommand{\sOR}{{\scriptscriptstyle \mathrm{OR}}}
\newcommand{\sB}{{\scriptscriptstyle \mathrm{OB}}}
\newcommand{\sD}{{\scriptscriptstyle \mathrm{D}}}
%\newcommand{\sR}{{\scriptscriptstyle \mathrm{R}}}
\newcommand{\sBB}{{\scriptscriptstyle \mathrm{BB}}}
\newcommand{\sBR}{{\scriptscriptstyle \mathrm{BR}}}
\newcommand{\sBL}{{\scriptscriptstyle \mathrm{BL}}}
\newcommand{\sBE}{{\scriptscriptstyle \mathrm{BE}}}
\newcommand{\sBA}{{\scriptscriptstyle \mathrm{BA}}}
\newcommand{\sblock}{{\scriptscriptstyle \mathrm{block}}}

\newcommand{\red}{\textcolor{red}}
\newcommand{\blue}{\textcolor{blue}}
%\newcommand{\violet}{\textcolor{violet}}


\newcommand\etal{\textit{et al.}}
\newcommand\ie{\textit{i.e.,}}
\newcommand\eg{\textit{e.g.,}}
\newcommand\wrt{\textit{w.r.t.}}
\newcommand\etc{\textit{etc.}}
\newcommand\iid{\textit{i.i.d.}}
\endinput

==> table_dataset.tex <==
\begin{table}[htbp]
  \centering  
  \begin{tabular}{c|ccccccccc}
  \toprule
  \toprule
    & Cham.
    & Squi.
    & Actor
    & Corn. 
    & Wisc. 
    & Texas  
    & Cora  
    & Cite.
    & Pubm.  \\
    
    \midrule
    \# Nodes 
    & 2,277
    & 5,201
    & 7,600
    & 183   
    & 251   
    & 183  
    & 2,708 
    & 3,327 
    & 19,717 \\
    
    \# Edges 
    & 36,101
    & 217,073
    & 33,544
    & 295   
    & 499   
    & 309  
    & 5,429 
    & 4,732 
    & 44,324 \\
    
    \# Features 
    & 2,325
    & 2,089
    & 931
    & 1,703 
    & 1,703 
    & 1,703 
    & 1,433 
    & 3,703
    & 500 \\
    
    \# Classes 
    & 5
    & 5
    & 5
    & 5     
    & 5     
    & 5    
    & 7     
    & 6
    & 3 \\
    
    $H_{\mathrm{node}}(G)^{\star}$
    & 0.23
    & 0.22
    & 0.22
    & 0.30
    & 0.21
    & 0.11
    & 0.81
    & 0.74
    & 0.80 \\
    
  \bottomrule
  \bottomrule
  \end{tabular}
  \caption{Benchmark dataset statistics. The $\star$ statistics are reported from \cite{ma2021homophily}.}
    
\end{table}


==> table_result.tex <==
%\begin{table}[htbp]
\begin{table}[t]
  \centering  
%   \tiny
%   \setlength{\tabcolsep}{0.5pt}
  \begin{tabular}{c|ccccccccc}
  \toprule
  \toprule
    & Cham.
    & Squi.
    & Actor
    & Corn. 
    & Wisc. 
    & Texas  
    & Cora  
    & Cite.
    & Pubm.  \\
    
    \midrule
    
    $\text{GAT}^{\dag}$  &
    42.93 &
    30.03 &
    28.45 & 
    54.32 & 
    49.41 & 
    58.38 & 
    86.37 &
    74.32 &
    87.62  \\
    
    $\text{DGN}^{\ddag}$  &
    50.48 &
    \cellcolor[rgb]{ .816,  .808,  .808}\textbf{37.46} &
    35.47 & 
    77.03 & 
    82.75 & 
    78.11 & 
    84.69 &
    73.87 &
    84.29  \\
    
    DGAT & 
    \cellcolor[rgb]{ .816,  .808,  .808}\textbf{52.47} &
    34.82 &
    \cellcolor[rgb]{ .816,  .808,  
    .808}\textbf{35.68} &
    \cellcolor[rgb]{ .816,  .808,  
    .808}\textbf{85.14} & 
    \cellcolor[rgb]{ .816,  .808,  
    .808}\textbf{84.71} & 
    \cellcolor[rgb]{ .816,  .808,  
    .808}\textbf{79.46} & 
    \cellcolor[rgb]{ .816,  .808,  .808}\textbf{88.05} & 
    \cellcolor[rgb]{ .816,  .808,  .808}\textbf{76.41}  &
    \cellcolor[rgb]{ .816,  .808,  .808}\textbf{87.93}
    \\
    
    \midrule
    $H_{\mathrm{node}}(\mathcal{G})$
    & 0.23
    & 0.22
    & 0.22
    & 0.30
    & 0.21
    & 0.11
    & 0.81
    & 0.74
    & 0.80 \\

  \bottomrule
  \bottomrule
  \end{tabular}
  \caption{Experimental results: average test accuracy (\%) of 9 real-world benchmark datasets. 
  The best results are highlighted. 
  Results "$\dag$" are reported from \cite{pei2020geom}. 
  Results "$\ddag$" are ran by searching the hyperparameters in the following ranges similar as Beaini et al.'s experimental setting \cite{beaini2021directional}: weight decay $\in [10^{-6}, 10^{-5}]$,
  learning rate $\in [10^{-5}, 10^{-4}]$,
  droupout ratio $\in [0.3, 0.5]$,
  aggreagators $\in\{$"mean-dir1-av", "mean-dir1-dx", "mean-dir1-av-dir1-dx"$\}$,
  net type $\in$ $\{$"complex", "simple"$\}$.
  For fair comparison, we use the same experimental setup as 
  \cite{pei2020geom},
  and report the average test accuracy over the same 10 fixed splits.}
  \label{table:real-res}
\end{table}

==> table_result_ablation.tex <==
% Table generated by Excel2LaTeX from sheet 'Results'
\begin{table*}[htbp]
% \hspace*{-1.2cm}
  \centering
  % \tiny
     \resizebox{1\hsize}{!}{
  \setlength{\tabcolsep}{1pt}
    \begin{tabular}{ccc|c|c|c|c|c|c|c|c|c}
    \toprule
   $\mathcal{R}(\mathcal{G})$%\tablefootnote{Neighour pruning} 
    & $\text{ATT}_\mathbf{e}$%\tablefootnote{Global directional aggregation} 
    & 
    $\mathbf{L}^{(\alpha, \gamma)}$%\tablefootnote{Parameterized random-walk Laplacian matrix} 
    & 
    chameleon & 
    squirrel & 
    actor  & 
    cornell & 
    wisconsin & 
    texas & 
    cora & 
    citeseer & 
    pubmed \\
    \midrule
    

    $\checkmark$ &       
    &      
    & 
    51.71 $\pm$ 1.23 &
    32.91 $\pm$ 2.26 & 
    35.24 $\pm$ 1.07 & 
    82.16 $\pm$ 5.94 &
    83.92 $\pm$ 3.59 & 
    78.38 $\pm$ 5.13 & 
    87.85 $\pm$ 1.02 & 
    74.50 $\pm$ 1.99 & 
    87.78 $\pm$ 0.44
    \\


    $\checkmark$ & 
    &
    $\checkmark$ &     
    
    51.91 $\pm$ 1.59 & 
    34.70 $\pm$ 1.02 &
    35.51 $\pm$ 0.74 &
    84.32 $\pm$ 4.15 & 
    84.12 $\pm$ 3.09 &
    78.65 $\pm$ 4.43 &
    87.83 $\pm$ 1.20 &
    76.18 $\pm$ 1.35 &
    87.93 $\pm$ 0.36 \\


    &       
    $\checkmark$ &      
    & 
    46.69 $\pm$ 1.98 &
    34.67 $\pm$ 0.10&
    29.63 $\pm$ 0.52 &
    60.27 $\pm$ 4.02 &
    54.51 $\pm$ 7.68 &
    60.81 $\pm$ 5.16 &
    87.95 $\pm$ 1.01 &
    76.31 $\pm$ 1.38 &
    87.90 $\pm$ 0.40 \\
    

    &       
    $\checkmark$ &      
    $\checkmark$ & 
    46.95 $\pm$ 2.50 &
    34.71 $\pm$ 1.02 &
    29.87 $\pm$ 0.60 &
    60.54 $\pm$ 0.40 &
    54.71 $\pm$ 5.68 &
    60.81 $\pm$ 4.87 &
    87.28 $\pm$ 1.53 &
    \textbf{76.41 $\pm$ 1.62} &
    87.88 $\pm$ 0.46 \\


    $\checkmark$ & 
    $\checkmark$ &       
    &     
    52.39 $\pm$ 2.08 &
    33.93 $\pm$ 1.86 &
    35.64 $\pm$ 0.10 &
    84.86 $\pm$ 5.12 &
    84.11 $\pm$ 2.69 &
    78.92 $\pm$ 5.57 &
    87.93 $\pm$ 0.99 &
    73.91 $\pm$ 1.62 &
    87.82 $\pm$ 0.30 \\


    $\checkmark$ & 
    $\checkmark$ &       
    $\checkmark$ &  
    \textbf{52.47 $\pm$ 1.44} &
    \textbf{34.82 $\pm$ 1.60} &
    \textbf{35.68 $\pm$ 1.20} &
    \textbf{85.14 $\pm$ 5.30} &
    \textbf{84.71 $\pm$ 3.59} &
    \textbf{79.46 $\pm$ 3.67} &
    \textbf{88.05 $\pm$ 1.09} &
    \textbf{76.41 $\pm$ 1.45} &
    \textbf{87.94 $\pm$ 0.48}
    \\

   \midrule
    &
    &
    &
    42.93 &
    30.03 &
    28.45 & 
    54.32 & 
    49.41 & 
    58.38 & 
    86.37 &
    74.32 &
    87.62  \\
   \bottomrule
   \end{tabular}%
   }
   \caption{Ablation study on 9 real-world datasets \cite{pei2020geom}. Cell with \checkmark means the component is applied to the DGAT model. The best test results are highlighted.}
   \label{tab:ablation_study}

\end{table*}
